Hybrid Memristor-CMOS (MeMOS) based Logic Gates and Adder Circuits

Practical memristor came into picture just few years back and instantly became the topic of interest for researchers and scientists. Memristor is the fourth basic two-terminal passive circuit element apart from well known resistor, capacitor and inductor. Recently, memristor based architectures has been proposed by many researchers. In this paper, we have designed a hybrid Memristor-CMOS (MeMOS) logic based adder circuit that can be used in numerous logic computational architectures. We have also analyzed the transient response of logic gates designed using MeMOS logic circuits. MeMOS use CMOS 180 nm process with memristor to compute boolean logic operations. Various parameters including speed, ares, delay and power dissipation are computed and compared with standard CMOS 180 nm logic design. The proposed logic shows better area utilization and excellent results from existing CMOS logic circuits at standard 1.8 V operating voltage.

==> images/iv1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(740,741){\makebox(0,0)[r]{\strut{}$-4.0$}}%
      \put(740,1370){\makebox(0,0)[r]{\strut{}$-2.0$}}%
      \put(740,2000){\makebox(0,0)[r]{\strut{}$0.0$}}%
      \put(740,2629){\makebox(0,0)[r]{\strut{}$2.0$}}%
      \put(740,3258){\makebox(0,0)[r]{\strut{}$4.0$}}%
      \put(951,440){\makebox(0,0){\strut{}$-1.0$}}%
      \put(1860,440){\makebox(0,0){\strut{}$-0.5$}}%
      \put(2770,440){\makebox(0,0){\strut{}$0.0$}}%
      \put(3679,440){\makebox(0,0){\strut{}$0.5$}}%
      \put(4588,440){\makebox(0,0){\strut{}$1.0$}}%
      \put(160,1999){\rotatebox{-270}{\makebox(0,0){\strut{}Current [mA]}}}%
      \put(2949,140){\makebox(0,0){\strut{}Voltage [V]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3732,1272){\makebox(0,0)[r]{\strut{}$\omega_{0}$}}%
      \csname LTb\endcsname%
      \put(3732,1072){\makebox(0,0)[r]{\strut{}$5\omega_{0}$}}%
      \csname LTb\endcsname%
      \put(3732,872){\makebox(0,0)[r]{\strut{}$10\omega_{0}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{images/iv1}}%
    \gplfronttext
  \end{picture}%
\endgroup

